Don't stop the training: continuously-updating self-supervised algorithms best account for auditory responses in the cortex

Over the last decade, numerous studies have shown that deep neural networks exhibit sensory representations similar to those of the mammalian brain, in that their activations linearly map onto cortical responses to the same sensory inputs. However, it remains unknown whether these artificial networks also learn like the brain. To address this issue, we analyze the brain responses of two ferret auditory cortices recorded with functional UltraSound imaging (fUS), while the animals were presented with 320 10\,s sounds. We compare these brain responses to the activations of Wav2vec 2.0, a self-supervised neural network pretrained with 960\,h of speech, and input with the same 320 sounds. Critically, we evaluate Wav2vec 2.0 under two distinct modes: (i) "Pretrained", where the same model is used for all sounds, and (ii) "Continuous Update", where the weights of the pretrained model are modified with back-propagation after every sound, presented in the same order as the ferrets. Our results show that the Continuous-Update mode leads Wav2Vec 2.0 to generate activations that are more similar to the brain than a Pretrained Wav2Vec 2.0 or than other control models using different training modes. These results suggest that the trial-by-trial modifications of self-supervised algorithms induced by back-propagation aligns with the corresponding fluctuations of cortical responses to sounds. Our finding thus provides empirical evidence of a common learning mechanism between self-supervised models and the mammalian cortex during sound processing.

==> figureTwo.tex <==

\begin{figure*}[ht]
% \vskip 0.2in
% \begin{center}
\centering
\centerline{\includegraphics[width=\linewidth]{figures/fig2.png}}
\caption{Continuously updated networks with backpropagation are more predictive of brain activity than frozen network. 
We report mean brain scores and standard error of the mean, with either an untrained network (no backprop), networks trained continuously with sounds presented in right order (same order as heard by the Ferret) or wrong order.
}
\label{fig:fig3}
% \end{center}
% \vskip -0.2in
\end{figure*}

% figure in supplementary
% \begin{figure}[ht]
% % \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{figures/figure_2bis.png}}
% \caption{Shuffle control: we repeat the experiment with 100 random order and compare the results to 3 run using the correct order but different (random) masking for the unsupervised loss computed at each sound. }
% \label{fig:fig4}
% \end{center}
% % \vskip -0.2in
% \end{figure}


\begin{figure}[ht]
% \vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\linewidth]{figures/fig3.png}}
\caption{Top, mean and standard error of the mean over all voxels in the different slices are shown. Bottom: each brain recording is repeated 4 times sequentially with different sounds order. Learning with the order of repetition X to predict the activity of a repetition Y (X $\neq$ Y) did not improve the brain score. }
\label{fig:fig4}
\end{center}
% \vskip -0.2in
\end{figure}


%old legend:
% Additional control. E



% \begin{figure}[ht]
% % \vskip 0.2in
% % \begin{center}
% \centering
% \centerline{\includegraphics[width=\linewidth]{figures/fig2ter.png}}
% \caption{ We separated the previous statistics over the different recording slices, gathering voxels in each slice separately. Color indicate a different brain hemisphere and experiment (N or V indicate experiment name, A or T the animal name, R or L the right or left hemisphere). Most of the slices presented significant results across the 3 random repetitions of the in silicon training. {\color{red} add stats} }
% \label{fig:fig2ter}
% % \end{center}
% % \vskip -0.2in
% \end{figure}



